Distributed State Machine Supervision for Long-baseline Gravitational-wave Detectors

The Laser Interferometer Gravitational-wave Observatory (LIGO) consists of two identical yet independent, widely-separated, long-baseline gravitational-wave detectors. Each Advanced LIGO detector consists of complex optical-mechanical systems isolated from the ground by multiple layers of active seismic isolation, all controlled by hundreds of fast, digital, feedback control systems. This article describes a novel state machine-based automation platform developed to handle the automation and supervisory control challenges of these detectors. The platform, called \textit{Guardian}, consists of distributed, independent, state machine automaton nodes organized hierarchically for full detector control. User code is written in standard Python and the platform is designed to facilitate the fast-paced development process associated with commissioning the complicated Advanced LIGO instruments. While developed specifically for the Advanced LIGO detectors, Guardian is a generic state machine automation platform that is useful for experimental control at all levels, from simple table-top setups to large-scale multi-million dollar facilities.

==> Makefile <==
DOC = paper
FIGS := \
	fig__ifo_glossary \
	fig__CDS-overview \
	fig__SUS-graph-path \
	fig__SUS-graph-jump \
	fig__H1-ISC_LOCK-hierarchy \
	fig__H1-SEI-hierarchy \
	fig__lock-acquisition \
	fig__sei-isolation \
	fig__flow_exit \
	fig__flow_continue \
	fig__flow_jump \
	fig__proc \
	example_system \

EXTRA = example_system.py
FILES = $(addsuffix .pdf, $(FIGS)) $(EXTRA)
TEX = $(DOC).tex
BIB = $(DOC).bib
AUX = $(DOC).aux
BBL = $(DOC).bbl
PDF = $(DOC).pdf
TGZ = $(DOC).tgz
ZIP = $(DOC).zip

DIST = $(TEX) $(BIB) $(BBL) $(FILES)

.PHONY: pdf
pdf: $(PDF)

$(AUX): $(TEX) $(FILES)
	pdflatex -halt-on-error $(DOC)
$(BBL): $(BIB) $(AUX)
	bibtex $(DOC)
$(PDF): $(BBL)
	pdflatex -halt-on-error $(DOC)
	pdflatex -halt-on-error $(DOC)

.PHONY: dist
dist: $(ZIP) $(TGZ)
$(ZIP): $(DIST)
	zip $@ $^ Makefile
$(TGZ): $(DIST)
	tar czf $@ $^ Makefile

.PHONY: clean
clean:
	rm -f *.aux *.bbl *.blg $(DOC)Notes.bib *.log *.out $(TGZ) $(ZIP)

